Context Embeddings for Efficient Answer Generation in RAG

Retrieval-Augmented Generation (RAG) allows overcoming the limited knowledge of LLMs by extending the input with external information. As a consequence, the contextual inputs to the model become much longer which slows down decoding time directly translating to the time a user has to wait for an answer. We address this challenge by presenting COCOM, an effective context compression method, reducing long contexts to only a handful of Context Embeddings speeding up the generation time by a large margin. Our method allows for different compression rates trading off decoding time for answer quality. Compared to earlier methods, COCOM allows for handling multiple contexts more effectively, significantly reducing decoding time for long inputs. Our method demonstrates a speed-up of up to 5.69 $\times$ while achieving higher performance compared to existing efficient context compression methods.

==> tables/main.tex <==
\begin{table*}[htb]
    \caption{Main Results comparing \acrs~to other RAG works. All methods use 5 context passages unless indicated otherwise. $^{\spadesuit}$ Based on Mistral-7B-v0.2. $^{\bigstar}$ Only compressor tuned. $^{\nabla}$ Method limited to single context.}
    \label{tab:main}
    \centering
    \small
    \setlength\tabcolsep{0pt} % let LaTeX figure out intecol. whitespace
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} lccccccccccc|cc}
\toprule
  \bfseries Model & \bfseries Compr. rate $\gamma$ & \multicolumn{2}{c}{\bfseries NQ} & \multicolumn{2}{c}{\bfseries TriviaQA} & \multicolumn{2}{c}{\bfseries HotpotQA} & \multicolumn{2}{c}{\bfseries ASQA} & \multicolumn{2}{c}{\bfseries PopQA} & \multicolumn{2}{c}{\bf Average}\\
  \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
    & & EM & M &EM & M &EM & M &EM & M &EM & M & EM & M\\
    \midrule
    % \textit{0-shot} & \\
    % RAG$^{\spadesuit}$ & \\
    % \multicolumn{1}{r}{w/ context} & \xmark &  0 & \\
    % \multicolumn{1}{r}{w/o context} & \xmark & 0 &  0.436\\
    % \midrule
     \textit{baseline}$^{\spadesuit}$  (no compr.)& \\
    \multicolumn{1}{r}{w/ RAG} & - & 0.597 &0.637 & 0.883 & 0.917 &0.500&0.544&0.622&0.665&0.513&0.543 & 0.623 & 0.661 \\
    \multicolumn{1}{r}{w/o RAG}& - & 0.362&0.403 & 0.708 & 0.753&0.264&0.283&0.546&0.573&0.199&0.208 & 0.416 & 0.444\\
    % Truncation &  & \\ 
    % Summarization  &  & \\ 
    % LLMlingual2 \cite{jiang-etal-2023-llmlingua} &   & \\ 
    AutoCompressor \cite{chevalier2023adapting}&  & \\
    ICAE \cite{ge2024incontext} $^{\bigstar}$& 4 &\\
    LloCo \cite{tan2024lloco} \\
    GridLM \cite{muennighoff2024generative} \\
    xRAG \cite{cheng2024xrag} $^{\bigstar, \nabla}$ & 128 & \\
   \multicolumn{1}{r}{Mistral-7B-v0.2} &  & 0.037 & 0.498 &0.142 &0.842 & 0.0336&0.366 & 0.050  & 0.514& 0.033 &0.399 & 0.059 & 0.524\\ 
    %\multicolumn{1}{r}{(30 tokens)}  &  & 0.037 & 0.412 &0.142 &0.804 & 0.0336&0.325 & 0.050  & 0.458& 0.033 &0.375\\     
    \multicolumn{1}{r}{Mixtral-8x7b}  &  & & & & & & & &\\ 
    \midrule
      \acrs-light$^{\spadesuit}$ \textit{(ours)} & 4 & 0.539&0.579&0.649&0.882&0.409&0.439&0.601&0.633&0.457&0.473 & 0.531 & 0.601\\ 
     & 16 & 0.492 & 0.529&0.823&0.857&0.367&0.395&0.565&0.604&0.385&0.395 & 0.526 & 0.556\\ 
     & 128 & 0.444 & 0.479 & 0.794 & 0.828 & 0.321&0.347&0.550&0.586 &0.314&0.326& 0.485 & 0.513\\ 
     \acrs$^{\spadesuit}$ \textit{(ours)} & 4 & 0.554&0.589&0.859&0.894&0.430&0.461&0.609&0.640&0.474&0.487 & 0.585 & 0.614\\ 
     & 16 &  0.539&0.577&0.852&0.886&0.426&0.456&0.602&0.633&0.465&0.478 & 0.577 & 0.606 \\ 
     & 128 & 0.511& 0.546&0.835&0.866&0.378&0.403&0.585&0.617&0.391&0.402 & 0.540 & 0.567\\ 

    \bottomrule
    \end{tabular*}
\end{table*}


==> tables/table1.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lcccccc}
        \toprule
     & num. emb. & Pre-training  & M & EM & Recall & LLMeval \\ 
        \midrule
        \textit{Baseline} \\ 
       tinyllama no retr. & \xmark & \xmark & 0.176 & 0.159 & 0.231 & \\
       tinyllama  & \xmark& \xmark &0.733 & 0.691 & 0.758 & \\
       \midrule
       \textit{Decoding from Embedding} \\ 
       
       
       
        tinyllama ae + tc  & 1 &100k steps &0.541 & 0.506 & 0.594 \\ %tc
        tinyllama ae +  me & 1 &100k steps & 0.533 & 0.500 & 0.592 \\
        tinyllama ae + tc + me & 1 &100k steps &0.536 & 0.499 & 0.594 \\ %tc + me
        \midrule
        tinyllama ae + tc  & 4 &50k steps & 0.579 &0.536  & 0.630\\  
        tinyllama ae +  me & 4 &50k steps &  0.556 & 0.521 & 0.638\\ 
        tinyllama ae + tc + me & 4 &50k steps &0.536 &0.499 &0.594 \\ 
        \bottomrule
    \end{tabular}
    \caption{Fine-tuning on NQ, num embs: 1, retrieval: 1. oracle document. 1 epoch, full ft, lr=5e-5}
    \label{tab:my_label}
\end{table}

==> tables/table2.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{lcccccc}
        \toprule
     & num. emb. & Pre-training  & M & EM & Recall & LLMeval \\ 
        \midrule
        \textit{Baseline} \\ 
       tinyllama no retr. & \xmark & \xmark & 0.176 & 0.159 & 0.231 & \\
       tinyllama  & \xmark& \xmark &0.733 & 0.691 & 0.758 & \\
       \midrule
       \textit{Decoding from Embedding} \\ 
       tinyllama  &1  & \xmark & 0.192 & 0.177 & 0.245 & \\
       tinyllama & 1 & 50k steps &  0.473 & 0.442 & 0.537 \\
       tinyllama  &  1&130k steps & 0.420 & 0.390 & 0.487 \\  
       tinyllama & 4 & 40k steps & 0.544 & 0.506 & 0.60 & \\
        \bottomrule
    \end{tabular}
    \caption{Fine-tuning on NQ, num embs: 1, retrieval: 1. oracle document. 1 epoch, full ft, lr=1e-4}
    \label{tab:my_label}
\end{table*}
